Variational Transfer Learning using Cross-Domain Latent Modulation

To successfully apply trained neural network models to new domains, powerful transfer learning solutions are essential. We propose to introduce a novel cross-domain latent modulation mechanism to a variational autoencoder framework so as to achieve effective transfer learning. Our key idea is to procure deep representations from one data domain and use it to influence the reparameterization of the latent variable of another domain. Specifically, deep representations of the source and target domains are first extracted by a unified inference model and aligned by employing gradient reversal. The learned deep representations are then cross-modulated to the latent encoding of the alternative domain, where consistency constraints are also applied. In the empirical validation that includes a number of transfer learning benchmark tasks for unsupervised domain adaptation and image-to-image translation, our model demonstrates competitive performance, which is also supported by evidence obtained from visualization.

==> appendices.tex <==
%\appendices

% \section{Supplementary}
\subsection{Reparameterization for Variational Cross-Domain Generation} \label{supp:repara-cross-domain}

In our model, the reparameterization can be written as follows:

\begin{equation}
  \begin{gathered}
    \bm{\ddot{z}}_{st} = \mathcal{G}((\bm \mu_s, \bm \sigma_s), \bm h_t) = \bm \mu_s + \bm \sigma_s \odot (\gamma_1\bm h_t + \gamma_2\bm \epsilon) \\
    \bm {\ddot{z}}_{ts} = \mathcal{G}((\bm \mu_t, \bm \sigma_t), \bm h_s) = \bm \mu_t + \bm \sigma_t \odot (\gamma_1\bm h_s + \gamma_2\bm \epsilon),
    \end{gathered}
    \label{eq:z_addition_appe}
\end{equation}
%where $i$ means the $i$th element. 
In general, consider $\bm h_s \sim p(\mathcal{H}_s) = \mathcal{N}(\bm \mu_{\bm h_s}, \bm \sigma_{\bm h_s})$, and $\bm h_t \sim p(\mathcal{H}_t) = \mathcal{N}(\bm \mu_{\bm h_t}, \bm \sigma_{\bm h_t})$. Adding the standard Gaussian distribution, $\epsilon \sim p(\epsilon) = \mathcal{N}(0, \mathbf{I})$, from Eq.(\ref{eq:z_addition_appe}) we have  $\bm{\ddot{z}}_{st} \sim \mathcal{N}(\bm{\ddot{z}}_{st}; \bm \mu_{st}, \bm \sigma_{st}^2\mathbf{I})$. The $i$-th element of its mean vector can be obtained as
\begin{equation}
\begin{split}
    \mu_{st}^i &= \mathbb{E}\{\mu^i_s + \sigma_s^i(\gamma_1 h_t^i + \gamma_2 \epsilon^i)\}\\
    & = \mu_s^i + \sigma_s^i\gamma_1 E\{h_t\} + \gamma_2 E\{\epsilon^i\} \\
    &= \mu_s^i + \gamma_1 \sigma_s^i \mu_{h_t}^i.
\end{split}
\end{equation}

Ignoring the bias term $\mu_s$, we have the $i$-th element of the variance vector:

\begin{equation}
    \begin{split}
        \mathbf{Var}(\ddot{z}_{st}^i) &= \mathbf{Var}[\sigma_s^i (\gamma_1 h_t^i + \gamma_2 \epsilon^i)]\\
        &=\mathbb{E}\{(\sigma_s^i(\gamma_1 h_t^i + \gamma_2\epsilon^i) - \gamma_1\sigma_s^i\mu_{h_t}^i)^2\} \\
        &= (\sigma_s^i)^2 \mathbb{E}\{[ (\gamma_1 h_t^i + \gamma_2\epsilon^i) - \gamma_1\mu_{h_t}^i]^2\} \\
        &= (\sigma_s^i)^2 \left( \mathbb{E}\{[ (\gamma_1 h_t^i + \gamma_2\epsilon^i)]^2\} - (\gamma_1 \mu_{h_t}^i)^2 \right) \\
        &= (\sigma_s^i)^2 [\gamma_1^2(\sigma_{h_t}^i)^2 + \gamma_2^2].
    \end{split}
\end{equation}
Therefore, the $i$-th element of the standard deviation vector $\bm\sigma_{st}$ is
\begin{equation}
    \sigma_{st}^i = \sigma_s^i \sqrt{\gamma_1^2(\sigma_{h_t}^i)^2 + \gamma_2^2}. 
\end{equation}

There is similar formulation for $\mu_{ts}^i$ and $\sigma_{ts}^i$, as follows:
\begin{equation}
\begin{gathered}
\mu_{ts}^i = \mu_t^i + \gamma_1 \sigma_t^i \mu_{h_s}^i \\
\sigma_{ts}^i = \sigma_t^i \sqrt{\gamma_1^2(\sigma_{h_s}^i)^2 + \gamma_2^2}
\end{gathered}
\end{equation} 



\subsection{Experiments Settings}
\label{supp:experiments_setting}
See Tables 5 -- 6.

\begin{table*}[]
    \centering
    \caption{Experiments Setting for Unsupervised Domain Adaptation}
    \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
            \hline
            \multirow{2}{*}{Experiments} & \multirow{2}{*}{enc\_style}  & \multirow{2}{*}{Encoder} & \multirow{2}{*}{Decoder} & \multirow{2}{*}{Discriminator} & \multicolumn{2}{|c|}{Encoder Updating} & \multicolumn{2}{|c|}{Decoder Updating} & \multicolumn{2}{|c|}{cls for pixel UDA}   \\
            \cline{6-11}
            &  &    &   &   & LR ($\eta_1$) & optimizer & LR ($\eta_2$) & optimizer &  LR & optimizer  \\
            \hline
            MNIST-MNISTM & fc (128*8)  & \makecell{f32k5s1-\\bn-\\f64k5s2-\\bn-\\f64k5s1-\\bn-\\f128k8s1-\\bn-\\f256k1s2-\\bn-\\f256k1s1}  & \makecell{f128k4s2-\\bn-\\f128k4s1-\\bn-\\f128k4s1-\\bn-\\f64k4s1-\\bn-\\f32k4s2-\\bn-\\f3k1s1}  & fc100-fc2  & \makecell{0.01\\annealing} & \makecell{Momentum-\\SGD (0.6)} & 0.0002  & \makecell{Adam \\($\beta_1$=0.5, \\ $\beta_2$=0.999)} & 0.001  & \makecell{Adam\\($\beta_1$=0.5,\\ $\beta_2$=0.999)}  \\
            \hline
            MNISTM-MNIST & fc (128*8) & - & - & - &\makecell{0.01\\annealing} & \makecell{Momentum-\\SGD (0.8)} & 0.2 & \makecell{Adam \\($\beta_1$=0.5, \\ $\beta_2$=0.999)} & 0.001 & \makecell{Adam\\($\beta_1$=0.5, \\ $\beta_2$=0.999)}  \\
            \hline
            MNIST-USPS & fc (128*8) & - & - & - &\makecell{0.01\\annealing} & \makecell{Momentum-\\SGD (0.8)} & 0.0002 & \makecell{Adam \\($\beta_1$=0.5, \\ $\beta_2$=0.999)} & 0.001 & \makecell{Adam\\($\beta_1$=0.5, \\ $\beta_2$=0.999)}  \\
            \hline
            USPS-MNIST & fc (128*8) & - & - & -  &\makecell{0.01\\annealing} & \makecell{Momentum-\\SGD (0.9)} & 0.001 & \makecell{Adam \\($\beta_1$=0.5, \\ $\beta_2$=0.999)} & 0.0008 & \makecell{Adam\\($\beta_1$=0.5, \\ $\beta_2$=0.999)}  \\
            \hline
            FASHION-FASHIONM & fc (128*8) & - & - & - &\makecell{0.01\\annealing} & \makecell{Momentum-\\SGD (0.8)} & 0.001 & \makecell{Adam \\($\beta_1$=0.5, \\ $\beta_2$=0.999)} & 0.001 & \makecell{Adam\\($\beta_1$=0.5, \\ $\beta_2$=0.999)}  \\
            \hline
            FASHIONM-FAHSION & fc (128*8) & -  & - & - &\makecell{0.01\\annealing} & \makecell{Momentum-\\SGD (0.9)} & 0.01 & \makecell{Adam \\($\beta_1$=0.5, \\ $\beta_2$=0.999)} & 0.001 & \makecell{Adam\\($\beta_1$=0.5, \\ $\beta_2$=0.999)}  \\
            \hline
            Linemod-linemod3D & fc (128*8) & - & - & - &\makecell{0.01\\annealing} & \makecell{Momentum-\\SGD (0.6)} & 2e-5 & \makecell{Adam \\($\beta_1$=0.5, \\ $\beta_2$=0.999)} & 0.0001 & \makecell{Adam\\($\beta_1$=0.5, \\ $\beta_2$=0.999)} \\
            \hline
    \end{tabular}}
\end{table*} 

\begin{table*}[]
    \centering
    \caption{Experiments Setting for Unsupervised Image Translation}
    \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
            \hline
            \multirow{2}{*}{Experiments} & \multirow{2}{*}{enc\_style}  & \multirow{2}{*}{Encoder} & \multirow{2}{*}{Decoder} & \multirow{2}{*}{Discriminator} & \multicolumn{2}{|c|}{Encoder Updating} & \multicolumn{2}{|c|}{Decoder Updating} \\
            \cline{6-9}
            &  &    &   &   & LR ($\eta_1$) & optimizer & LR ($\eta_2$) & optimizer \\
            \hline
            Shoes-edge & fc (128*8)  & \makecell{f32k5s1-\\bn-\\f64k5s2-\\bn-\\f64k5s1-\\bn-\\f128k8s1-\\bn-\\f256k1s2-\\bn-\\f256k1s1} & \makecell{f128k4s2-\\bn-\\f128k4s1-\\bn-\\f128k4s1-\\bn-\\f64k4s1-\\bn-\\f32k4s2-\\bn-\\f3k1s1} & fc100-fc2  & \makecell{0.01\\annealing} & \makecell{Momentum-\\SGD (0.4)} & 0.002  & \makecell{Adam \\($\beta_1$=0.5, \\ $\beta_2$=0.999)}  \\
            \hline
            edge-Shoes & fc (128*8) & - & - & -  &\makecell{0.01\\annealing} & \makecell{Momentum-\\SGD (0.6)} & 0.02 & \makecell{Adam \\($\beta_1$=0.5, \\ $\beta_2$=0.999)} \\
            \hline
            CelebA-Sketched CelebA & fc (128*8) & - & - & -  &\makecell{0.01\\annealing} & \makecell{Momentum-\\SGD (0.6)} & 0.2 & \makecell{Adam \\($\beta_1$=0.5, \\ $\beta_2$=0.999)}  \\
            \hline
            Sketched CelebA-CelebA & fc (128*8) & - & - & -   &\makecell{0.01\\annealing} & \makecell{Momentum-\\SGD (0.6)} & 0.2 & \makecell{Adam \\($\beta_1$=0.5, \\ $\beta_2$=0.999)}  \\
            \hline
    \end{tabular}}
\end{table*}

\subsection{More Generation Images}
\label{supp:more_generations}
See Figures 8 -- 18.

\begin{figure*}[thbp]
   \centering
   \includegraphics[width=1.0\textwidth]{exp_mnist_mnistm_more_imgs}
   \caption{More Generations in task MNIST(source)-MNISTM(target)}
   \label{fig:mnist_mnistm_more}
\end{figure*}

\begin{figure*}[thbp]
   \centering
   \includegraphics[width=1.0\textwidth]{exp_mnistm_mnist_more_imgs}
   \caption{More Generations in task MNISTM(source) -- MNIST(target)}
   \label{fig:mnistm_mnist_more}
\end{figure*}

\begin{figure*}[thbp]
   \centering
   \includegraphics[width=1.0\textwidth]{exp_mnist_usps_more_imgs}
   \caption{More Generations in task MNIST(source) -- USPS(target)}
   \label{fig:mnist_usps_more}
\end{figure*}

\begin{figure*}[thbp]
   \centering
   \includegraphics[width=1.0\textwidth]{exp_usps_mnist_more_imgs}
   \caption{More Generations in task USPS(source) -- MNIST(target)}
   \label{fig:usps_mnist_more}
\end{figure*}

\begin{figure*}[thbp]
   \centering
   \includegraphics[width=1.0\textwidth]{exp_fashion_fashionm_more_imgs}
   \caption{More Generations in task Fashion(source) -- FashionM(target)}
   \label{fig:fashion_fashionm_more}
\end{figure*}

\begin{figure*}[thbp]
   \centering
   \includegraphics[width=1.0\textwidth]{exp_fashionm_fashion_more_imgs}
   \caption{More Generations in task FashionM(source) -- Fashion(target)}
   \label{fig:fashionm_fashion_more}
\end{figure*}

\begin{figure*}[thpb]
   \centering
   \includegraphics[width=1.0\textwidth]{exp_linemod_more_imgs}
   \caption{More Generations in task Linemod3D(source) -- LinemodReal(target)}
   \label{fig:linemod_more}
\end{figure*}

\begin{figure*}[thbp]
   \centering
   \includegraphics[width=1.0\textwidth]{exp_edge_shoes_more_imgs}
   \caption{More Generations in task Shoes(source) -- edge(target)}
   \label{fig:shoes_edge_more}
\end{figure*}

\begin{figure*}[thbp]
   \centering
   \includegraphics[width=1.0\textwidth]{exp_shoes_edge_more_imgs}
   \caption{More Generations in task edge(source) -- Shoes(target)}
   \label{fig:edge_shoes_more}
\end{figure*}

\begin{figure*}[thbp]
   \centering
   \includegraphics[width=1.0\textwidth]{exp_sketch_face_more_imgs}
   \caption{More Generations in task CelebA(source) -- Sketch(target)}
   \label{fig:face_sketch_more}
\end{figure*}

\begin{figure*}[thbp]
   \centering
   \includegraphics[width=1.0\textwidth]{exp_face_sketch_more_imgs}
   \caption{More Generations in task Sketch(source) -- CelebA(target)}
   \label{fig:sketch_face_more}
\end{figure*}

